An Analysis of Super-Net Heuristics in Weight-Sharing NAS

Weight sharing promises to make neural architecture search (NAS) tractable even on commodity hardware. Existing methods in this space rely on a diverse set of heuristics to design and train the shared-weight backbone network, a.k.a. the super-net. Since heuristics substantially vary across different methods and have not been carefully studied, it is unclear to which extent they impact super-net training and hence the weight-sharing NAS algorithms. In this paper, we disentangle super-net training from the search algorithm, isolate 14 frequently-used training heuristics, and evaluate them over three benchmark search spaces. Our analysis uncovers that several commonly-used heuristics negatively impact the correlation between super-net and stand-alone performance, whereas simple, but often overlooked factors, such as proper hyper-parameter settings, are key to achieve strong performance. Equipped with this knowledge, we show that simple random search achieves competitive performance to complex state-of-the-art NAS algorithms when the super-net is properly trained.

==> figure/lowfidelity-nb102.tex <==
% \begin{figure}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \includegraphics{figsourse/batch-size-nasbench102.pdf}
%     }
%     \vspace{-0.8cm}
%     \caption{\textbf{Reducing batch-size on NASBench-201} with 400 epochs. Note that reducing the batch-size will slightly reduce the final model performances as well as the super-net ranking performance.}
%     \label{fig:lr-nasbench201}
% \end{figure}

\begin{figure}[t]
    \centering
    \vspace{-0.2cm}
    \resizebox{\linewidth}{!}{
    \includegraphics{figsourse/low-fidelity-horizontal.pdf}
    }\vspace{-0.2cm}
    \caption{\textbf{Low fidelity estimates on NASBench-201.} 
    From top-left in clock-wise order: batch-size, number of repeated cells, number of channels, and portion of training data. Reducing batch-size or the number of channels negatively impacts performance, whereas a reduced number of cells or a smaller training set have limited influence.
    % \KY{too red for portion plot, need to set alpha for that...}
    % \KY{increase the resolution for middle graph. add p $>$ r into middle graph.v}
    }
    \vspace{-0.7cm}
    \label{fig:low-fidelity}
\end{figure}



==> figure/lowfidelity-reduce.tex <==
% \begin{wrapfigure}{r}{0.33\linewidth}
%     \centering
%         \vspace{-.4cm}
%     \resizebox{\linewidth}{!}{
%     \includegraphics{figsourse/low-fidelity-reduce.pdf}
%     }
%     \vspace{-0.7cm}
%     \caption{Low fidelity estimates on NASBench-201. 
%     % \KY{fix legend of BS}
%     }
%     \vspace{-0.4cm}
%     \label{fig:low-fidelity}
% \end{wrapfigure}


==> figure/lr-other-spaces.tex <==
% \begin{wrapfigure}{r}{0.5\linewidth}
%     \vspace{-1cm}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \includegraphics{figsourse/validate-learning_ratenasbench101.pdf}
%     }
%     \vspace{-0.7cm}
%     \caption{\textbf{Learning rate} on NASBench-101.}
%     \label{fig:supp:lr-nasbench101}
%     % \vspace{0.2cm}
%     \hfill
%     \resizebox{\linewidth}{!}{
%     \includegraphics{figsourse/validate-learning_ratedarts_nds.pdf}
%     }
%     \vspace{-0.7cm}
%     \caption{\textbf{Learning rate} on DARTS-NDS.}
%     \label{fig:supp:lr-darts-nds}
%     \vspace{-0.3cm}
% \end{wrapfigure}

\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics{figsourse/validate-learning_ratenasbench101.pdf}
    }
    \resizebox{\linewidth}{!}{
    \includegraphics{figsourse/validate-learning_ratedarts_nds.pdf}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Learning rate} on NASBench-101 (Top) and DARTS-NDS (Bottom).}
    \label{fig:supp:lr-other}
\end{figure}

% \begin{figure*}
%     \centering
%     \begin{minipage}{0.48\linewidth}
%     \resizebox{\linewidth}{!}{
%     \includegraphics{figsourse/validate-learning_ratenasbench101.pdf}
%     }
%     \vspace{-0.7cm}
%     \caption{\textbf{Learning rate} on NASBench-101.}
%     \label{fig:supp:lr-nasbench101}
%     \end{minipage}
%     % \vspace{0.2cm}
%     \hfill
%     \begin{minipage}{0.48\linewidth}
%     \resizebox{\linewidth}{!}{
%     \includegraphics{figsourse/validate-learning_ratedarts_nds.pdf}
%     }
%     \vspace{-0.2cm}
%     \caption{\textbf{Learning rate} on DARTS-NDS.}
%     \label{fig:supp:lr-darts-nds}
%     \end{minipage}
% \end{figure*}

==> figure/nb101-linear.tex <==
\begin{figure}
    \centering
        % \vspace{-.4cm}
    \resizebox{0.7\linewidth}{!}{
    \includegraphics{figsourse/nb101-linear.pdf}
    }
    \caption{\textbf{Simplifying NASBench-101 to a linear search space.} (a) The original NASBench-101 is a general direct acyclic graph (DAG) search space that each node can be connected to all previous nodes. (b) To mimic a linear search space like MobileNet~\cite{wu_fbnet:_2018} we ensure that each node is only connected to its predecessor. As a consequence, the search is reduced only to operations for each node. This toy search space has 243 architectures in total. 
    }
    \vspace{-0.4cm}
    \label{fig:nb101-linear}
\end{figure}


==> figure/sota-correlation.tex <==
\begin{figure}[!b]
% \begin{minipage}[t]{\textwidth}
    \centering
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \vspace{-0.4cm}
        \resizebox{\linewidth}{!}{
        \hspace{-1.cm}
        \includegraphics{figsourse/supernet-evaluation.pdf}
        }
        \resizebox{0.8\linewidth}{!}{
        \begin{tabular}{l|ccc}
        Spearman Corr.     &  Acc. - Perf. & S-KdT - Perf. & Acc. - S-KdT \\
        \midrule
        NASBench-101 & 0.09  & 0.45 & 0.23 \\
        NASBench-201 & 0.52  & 0.55 & 0.94 \\
        DARTS-NDS    & 0.07  & 0.19 & 0.47 \\
        \end{tabular}}
        % \vspace{-0.2cm}
        \captionof{figure}{\textbf{Super-net evaluation}. We collect all experiments across 3 benchmark spaces. \textbf{(Top)} Pairwise plots of super-net accuracy, final performance, and the \skdt{}. Each point corresponds to to one individual evaluation of the super-net. \textbf{(Bottom)} Spearman correlation coefficients between the metrics.
        }
        % \vspace{-0.3cm}
        \label{fig:supernet}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \vspace{-0.4cm}
        \captionof{table}{
        \textbf{Search results on 3 search spaces.} 
        % \textbf{Search results on CIFAR-10 across spaces.} 
        Results on NASBench-101 and NASBench-201 are taken from \citet{yu2020evalnas}, and \citet{dong2020bench102}. We report the mean ($\pm$ std) over 3 different runs. Note that NASBench-101 (n=7) in \citep{yu2020evalnas} is identical to our setting. Our new strategy significantly surpasses the random search baseline.
        }
        \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cccc}
        \toprule
             Method &  NASBench & NASBench & DARTS & DARTS \\
             & 101 & 201 & NDS & NDS$^\star$ \\
             \midrule
             ENAS & 91.83 $\pm$ 0.42 & 54.30 $\pm$ 0.00  & 94.45& 97.11 \\
             DARTS-V2 & 92.21 $\pm$ 0.61 & 54.30 $\pm$ 0.00 & 94.79 & 97.37 \\
             NAO  & 92.59 $\pm$ 0.59 & - & - & 97.10 \\
             GDAS & - & 93.51 $\pm$ 0.13 & - & 96.23 \\
             \midrule 
              Random NAS & 89.89 $\pm$ 3.89 & 87.66 $\pm$ 1.69 & 91.33 & 96.74$^\dag$ \\
             Random NAS (Ours) & 93.12 $\pm$ 0.06 & 92.90 $\pm$ 0.14 & 94.26 $\pm$ 0.05 & 97.08 \\
             \bottomrule
             \multicolumn{5}{l}{$^{\dag}$Result took from \citet{li2019random}} \\
             \multicolumn{5}{l}{$^{\star}$Trained according to \citet{Liu2018darts} for 600 epochs.} \\
             \multicolumn{5}{l}{DARTS-V2~\citep{Liu2018darts}, ENAS~\citep{Pham2018},NAO~\citep{Luo2018}.} \\
             \multicolumn{5}{l}{Random-NAS~\citep{li2019random},GDAS~\citep{dong2019searching}} \\
        \end{tabular}
        }
        \label{tab:sota}
        % \vspace{-0.5cm}
    \end{minipage}
\vspace{-0.6cm}
% \end{minipage}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> table/hp-epochs.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular} { lcccc c cccc c cccc c  }
\toprule
&\multicolumn{4}{c}{nasbench101} &&\multicolumn{4}{c}{nasbench102} &&\multicolumn{4}{c}{darts-nds} &\\
\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}
Epochs & 100 & 200 & 300 & 400&& 100 & 400 & 1200 & 1800&& 100 & 200 & 300 & 400&\\
Kd-T & 0.159 & 0.137 & 0.223 & 0.123 & & 0.331 & 0.633 & 0.667 & 0.681 & & 0.114 & 0.144 & 0.123 & 0.136 & \\
P > R & 0.81 & 0.81 & 0.81 & 0.80 & & 1.00 & 0.93 & 0.68 & 0.71 & & 0.79 & 0.71 & 0.17 & 0.17 & \\
Acc. & 46.78 $\pm$ 0.00 & 66.20 $\pm$ 0.00 & 72.73 $\pm$ 0.00 & 77.10 $\pm$ 0.00 & & 47.17 $\pm$ 0.34 & 69.68 $\pm$ 1.80 & 77.54 $\pm$ 0.00 & 78.30 $\pm$ 0.00 & & 64.28 $\pm$ 0.82 & 76.09 $\pm$ 0.36 & 79.25 $\pm$ 2.97 & 79.79 $\pm$ 5.23 & \\
    \bottomrule
    \end{tabular}
    }
    \caption{\bf{Validating the number of epochs across benchmark datasets.} }
    \label{tab:hp-epochs}
\end{table*}

==> table/hp-initial-channels.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular} { lcccc c cccc c cccc c  }
\toprule
&\multicolumn{4}{c}{nasbench101} &&\multicolumn{4}{c}{nasbench102} &&\multicolumn{4}{c}{darts-nds} &\\
\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}
Epochs & 100 & 200 & 300 & 400&& 100 & 400 & 1200 & 1800&& 100 & 200 & 300 & 400&\\
Kd-T & 0.159 & 0.137 & 0.223 & 0.123 & & 0.331 & 0.633 & 0.667 & 0.681 & & 0.114 & 0.144 & 0.123 & 0.136 & \\
P > R & 0.81 & 0.81 & 0.81 & 0.80 & & 1.00 & 0.93 & 0.68 & 0.71 & & 0.79 & 0.71 & 0.17 & 0.17 & \\
Acc. & 46.78 $\pm$ 0.00 & 66.20 $\pm$ 0.00 & 72.73 $\pm$ 0.00 & 77.10 $\pm$ 0.00 & & 47.17 $\pm$ 0.34 & 69.68 $\pm$ 1.80 & 77.54 $\pm$ 0.00 & 78.30 $\pm$ 0.00 & & 64.28 $\pm$ 0.82 & 76.09 $\pm$ 0.36 & 79.25 $\pm$ 2.97 & 79.79 $\pm$ 5.23 & \\
    \bottomrule
    \end{tabular}
    }
    \caption{\bf{Validating the number of epochs across benchmark datasets.} }
    \label{tab:hp-epochs}
\end{table*}

==> table/hp-low-fiedality-all.tex <==


% \begin{table*}[h]
%     \centering
%     \resizebox{\linewidth}{!}{
% \begin{tabular} { llccc l ccc l ccc l  }
% &&\multicolumn{3}{c}{NASBench-101}&&\multicolumn{3}{c}{NASBench-201}&&\multicolumn{3}{c}{DARTS-NDS}&\\
% \cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-13}
% &&Kd-T&Acc.&Best&&Kd-T&Acc.&Best&&Kd-T&Acc.&Best&\\
% \midrule
% B&& 0.75 &0.7586913832880819&&0.66 $\pm 0.07&0.71 $\pm 0.15&0.851669222656049&&0.17 $\pm 0.01&0.71 $\pm 0.06&0.8803196887040001&\\
% B/2&&0.24 $\pm 0.02&0.67 $\pm 0.05&0.9230784004206745&&0.65 $\pm 0.05&0.71 $\pm 0.15&0.6346617234268707&&0.18 $\pm 0.04&0.72 $\pm 0.07&0.8803196887040001&\\
% B/4&&0.15 $\pm 0.02&0.69 $\pm 0.07&0.9758918003530775&&0.62 $\pm 0.03&0.70 $\pm 0.15&0.8290057835878809&&0.13 $\pm 0.02&0.71 $\pm 0.09&0.8803196887040001&\\
% \bottomrule
% \end{tabular}

% }
%     \caption{\bf{Low fidelity estimates results.} 
%     \KY{Note that, the Portion for DARTS-NDS is with affine=True. redo now!}}
%     \label{tab:hp-low-fidelity-all}
% \end{table*}


\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{
\begin{tabular} { llcc l cc l cc l  }
\toprule
&&\multicolumn{2}{c}{NASBench-101}&&\multicolumn{2}{c}{NASBench-201}&&\multicolumn{2}{c}{DARTS-NDS}&\\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
&&Kd-T&Acc.&&Kd-T&Acc.&&Kd-T&Acc.&\\
\midrule
Baseline &&0.19&0.69&&0.73&0.71&&0.18&0.71&\\
\midrule
B/2&&0.20&0.70&&0.65&0.70&&0.17&0.72&\\
B/4&&0.16&0.77&&0.62&0.72&&0.16&0.71&\\
\midrule
L-1&&0.15&0.76&&0.66&0.75&&0.15&0.84&\\
L-2&&0.13&0.82&&0.67&0.78&&0.15&0.85&\\
L-3&&-&-&&0.61&0.78&&0.12&0.85&\\
\midrule
P=0.9&&0.19&0.77&&0.66&0.77&&0.04&0.40&\\
P=0.75&&0.30&0.74&&0.67&0.76&&0.04&0.34&\\
P=0.5&&0.24&0.67&&0.64&0.74&&0.04&0.28&\\
P=0.25&&0.28&0.48&&0.60&0.66&&0.03&0.42&\\
\midrule
C/2&&-&-&&0.59&0.60&&0.17&0.78& \\
C/4&&-&-&&0.54&0.45&&0.15&0.71&\\
\bottomrule
\end{tabular}
}
    \caption{\bf{Low fidelity estimates results.} 
    \KY{Note that, the Portion for DARTS-NDS is with affine=True. redo now!}}
    \label{tab:hp-low-fidelity-all}
\end{table}



==> table/huge-nb101-chain.tex <==
\begin{table}[!ht]
    \centering
    \caption{\textbf{Results for all WS Protocol $P_{ws}$ factors on the NASBench-101 linear space.}} 
    \vspace{-0.3cm}
    \resizebox{\linewidth}{!}{
        \begin{tabular} { l|cccc}
        \midrule[2pt]
        Factor & \multicolumn{4}{c}{NASBench-101 linear space} \\
        and &  & Super-net & & Final \\
        settings & Accuracy & S-KdT & P $>$ R &  Performance\\
        \midrule[1pt]
        \multicolumn{3}{l}{\textbf{Batch-norm}} \\
        \midrule
affine F track F &0.478$\pm$0.04&0.131&0.960&0.866$\pm$0.01\\
affine T track F &0.487$\pm$0.07&0.146&0.542&0.852$\pm$0.02\\
affine F track T &0.103$\pm$0.01&-0.154&0.263&0.855$\pm$0.01\\
affine T track T &0.111$\pm$0.02&-0.121&0.651&0.857$\pm$0.01\\
        \midrule[1pt]
        \multicolumn{3}{l}{\textbf{Learning rate}} \\
        \midrule
0.001 &0.188$\pm$0.08&0.363&0.636&0.869$\pm$0.01\\
0.005 &0.515$\pm$0.09&0.558&0.828&0.867$\pm$0.01\\
0.01 &0.570$\pm$0.03&0.233&0.920&0.853$\pm$0.02\\
0.025 &0.568$\pm$0.05&0.160&0.194&0.848$\pm$0.01\\
0.1 &0.655$\pm$0.05&0.168&0.696&0.860$\pm$0.02\\
0.15 &0.593$\pm$0.05&0.148&0.256&0.822$\pm$0.05\\
        \midrule[1pt]
        \multicolumn{4}{l}{\textbf{Epochs}} \\
        \midrule
200 &0.235$\pm$0.02&0.004&0.696&0.861$\pm$0.01\\
300 &0.397$\pm$0.03&0.118&0.960&0.849$\pm$0.04\\
400 &0.508$\pm$0.05&0.114&0.810&0.837$\pm$0.03\\
800 &0.741$\pm$0.04&0.232&0.846&0.860$\pm$0.02\\
1000 &0.775$\pm$0.04&0.216&0.568&0.851$\pm$0.02\\
        \midrule[1pt]
        \multicolumn{4}{l}{\textbf{Weight decay} } \\
        \midrule
        0.0 &0.429$\pm$0.03&0.151&0.300&0.830$\pm$0.03\\
0.0001 &0.563$\pm$0.05&0.134&0.449&0.856$\pm$0.01\\
0.0003 &0.639$\pm$0.05&0.170&0.188&0.841$\pm$0.02\\
0.0005 &0.697$\pm$0.04&0.198&0.124&0.842$\pm$0.01\\
        \midrule[2pt]
        \end{tabular}
}
\label{tab:pws-nasbench101-linear}
\end{table}

\begin{table}[!ht]
% here is the low fidality 
	\caption{\textbf{Results for all low-fidelity factors on the three search spaces.}} 
	\vspace{-0.3cm}
\resizebox{\linewidth}{!}{
	\begin{tabular} { l|cccc}
        \midrule[2pt]
		Factor & \multicolumn{4}{c}{NASBench-101 Chain-like Space} \\
		and & Super-net & \phantom{0} & \phantom{0} & Final \\
		settings & Accuracy & S-KdT & P $>$ R &  Performance \\
        \midrule[1pt]
		\multicolumn{5}{l}{\textbf{Number of layers} (-X indicates the baseline minus X)} \\
		\midrule
Baseline &0.543$\pm$0.05&0.126&0.555&0.863$\pm$0.01\\
-1 &0.734$\pm$0.03&0.184&0.324&0.858$\pm$0.01\\
-2 &0.813$\pm$0.03&0.184&0.270&0.847$\pm$0.02\\
        \midrule[1pt]
		\multicolumn{3}{l}{\textbf{Train portion}} \\
		\midrule
0.25 &0.222$\pm$0.01&0.105&0.542&0.845$\pm$0.02\\
0.5 &0.358$\pm$0.02&0.093&0.696&0.862$\pm$0.01\\
0.75 &0.341$\pm$0.04&0.055&0.308&0.853$\pm$0.01\\
0.9 &0.518$\pm$0.05&0.114&0.136&0.847$\pm$0.01\\        
\midrule[1pt]
		\multicolumn{5}{l}{\textbf{Batch size} (/ X indicates the baseline divided by X)} \\
		\midrule
Baseline &0.566$\pm$0.05&0.158&0.864&0.861$\pm$0.01\\
/2 &0.621$\pm$0.05&0.124&0.920&0.870$\pm$0.01\\
/4 &0.639$\pm$0.06&0.183&0.494&0.848$\pm$0.01\\
        \midrule[1pt]
		\multicolumn{5}{l}{\textbf{\# channels} (/ X indicates the baseline divided by X)} \\
		\midrule
Baseline &0.561$\pm$0.05&0.146&0.864&0.866$\pm$0.01\\
/2 &0.554$\pm$0.05&0.158&0.407&0.843$\pm$0.02\\
/4 &0.435$\pm$0.03&0.153&0.102&0.826$\pm$0.04\\
        \midrule[2pt]
	\end{tabular}
}
\label{tab:supp-lowfd-nb101-linear}
\end{table}



==> table/other-fws.tex <==

\begin{table}
\caption{\textbf{Comparison of different mappings $f_{ws}$}. 
%We compare weight-sharing batch-norm~(WSBN), projecting operation on the node (Node) or on the edge (Edge), as well as sharing the convolutional kernels as in~\cite{Cai2020Once}~(OFA). 
We report s-KdT $/$ final search performance.}
    \centering
    \resizebox{0.9\linewidth}{!}{
        \begin{tabular} { l|ccc}
\toprule
& NASBench-101 & NASBench-201 & DARTS-NDS \\
\midrule
\midrule
Baseline          & 0.236 $/$ 92.32    & 0.740 $/$ 92.92    & 0.159 $/$ 93.59 \\
\midrule
WSBN              & 0.056 $/$ 91.33    & 0.675 $/$ 92.04  & 0.331 $/$ 92.95 \\
Global-Dropout    & 0.179 $/$ 90.95     & 0.676 $/$ 91.76   & 0.102 $/$ 92.30 \\
Path-Dropout      & 0.128 $/$ 91.19     & 0.431 $/$ 91.42   & 0.090 $/$ 91.90 \\
% \midrule
% Op-Edge           & N/A & as Baseline   & 0.189 $/$ 93.97 \\
% Op-Node           & as Baseline         & 0.738 $/$ 92.36   & as Baseline \\
\midrule
OFA Kernel        & 0.132 $/$ 92.01    & 0.574 $/$ 91.83  & 0.112 $/$ 92.83 \\
\bottomrule
\end{tabular}
}
% \vspace{-0.2cm}
\label{tab:hp-fws}
\end{table}

% \begin{table}[t]
%     \centering
%     \begin{minipage}{0.48\linewidth}
%         \vspace{0.2cm}
%     \caption{\textbf{Disabling dynamic channels}} 
%     \resizebox{0.95\linewidth}{!}{
%         \begin{tabular} { l|cccc}
%         \toprule
%         Edges & Accuracy & S-KdT & P $>$ R & Final searched model \\
%         \midrule
%         \multicolumn{5}{l}{\textit{Baseline: random sampling sub-spaces with dynamic channeling.}} \\
% 1 &70.04$\pm$\phantom{0}8.15&0.173&0.797&91.19$\pm$2.01\\
% 2 &78.29$\pm$10.51&0.206&0.734&82.03$\pm$1.50\\
% 3 &79.92$\pm$\phantom{0}9.42&0.242&0.576&92.20$\pm$1.19\\
% 4 &79.37$\pm$\phantom{0}17.34&0.270&0.793&92.32$\pm$1.10\\
% \midrule
% Average       & 76.905 $\pm$ 10.05 & 0.223 & 0.865 & 89.435 $\pm$ 4.30 \\
%         \midrule
%         \midrule
%         \multicolumn{5}{l}{\textit{Disable dynamic channels by fixing the edges to the output node.}} \\
% 1 &76.92$\pm$\phantom{0}7.87&0.435&0.991&93.94$\pm$0.22\\
% 2 &74.32$\pm$\phantom{0}8.21&0.426&0.925&93.34$\pm$0.01\\
% 3 &77.24$\pm$\phantom{0}9.18&0.487&0.901&93.66$\pm$0.07\\
% 4 &79.31$\pm$\phantom{0}7.04&0.493&0.978&93.65$\pm$0.07\\
% \midrule
%         Average       & 76.95 $\pm$ \phantom{0}8.29 & 0.460 & 0.949 & 93.65 $\pm$ 0.73 \\
%         \bottomrule
%         \end{tabular}
%     }
%     \label{tab:disable-dynamic-channel-results}
%     \end{minipage}
%     % \vspace{0.2cm}
%     \hfill
%     \begin{minipage}{0.48\linewidth}
%     \vspace{-0.9cm}
% \caption{\textbf{Comparison of different mappings $f_{ws}$}. 
% %We compare weight-sharing batch-norm~(WSBN), projecting operation on the node (Node) or on the edge (Edge), as well as sharing the convolutional kernels as in~\cite{Cai2020Once}~(OFA). 
% We report s-KdT $/$ final search performance.}
%     \centering
%     \resizebox{0.9\linewidth}{!}{
%         \begin{tabular} { l|ccc}
% \toprule
% & NASBench-101 & NASBench-201 & DARTS-NDS \\
% \midrule
% \midrule
% Baseline          & 0.236 $/$ 92.32    & 0.740 $/$ 92.92    & 0.159 $/$ 93.59 \\
% \midrule
% WSBN              & 0.056 $/$ 91.33    & 0.675 $/$ 92.04  & 0.331 $/$ 92.95 \\
% Global-Dropout    & 0.179 $/$ 90.95     & 0.676 $/$ 91.76   & 0.102 $/$ 92.30 \\
% Path-Dropout      & 0.128 $/$ 91.19     & 0.431 $/$ 91.42   & 0.090 $/$ 91.90 \\
% % \midrule
% % Op-Edge           & N/A & as Baseline   & 0.189 $/$ 93.97 \\
% % Op-Node           & as Baseline         & 0.738 $/$ 92.36   & as Baseline \\
% \midrule
% OFA Kernel        & 0.132 $/$ 92.01    & 0.574 $/$ 91.83  & 0.112 $/$ 92.83 \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-0.2cm}
% \label{tab:hp-fws}
%     \end{minipage}
% \end{table}

% \begin{wraptable}{r}{0.2\linewidth}
% \begin{table}
% % \vspace{-0.4cm}
%     \centering
%         \captionof{table}{NASBench-101 sub-spaces obtained by fixing the number of channels.}
%         \vspace{-0.2cm}
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{c|c}
%     \toprule
%     \# Incoming     & \# Arch.  \\
%      Edge &\\
%     \midrule
%     1 &  120933 \\
%     2 & 201441 \\
%     3 & 90782 \\
%     4 & 10467 \\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:disable-channel}
% \end{table}
% \vspace{-0.7cm}
% \end{wraptable}


==> tex/R1.tex <==
\section{Reviewer 1}

\mypara{Q1.} \textit{Why not include non-cell-structure search space (i.e., chain-like search space without topology) for extensive study (e.g., FairNAS, MobileNet-like) ? I strongly encourage the authors to consider this, which would benefit the area more.}

\mypara{Reply:} Our extensive evaluation critically requires access to the performance of a significant subset of architectures of a given search space which have been trained in a stand-alone fashion. As such we rely on the NASBench series of works, which provide thousands of trained architectures together with their performance for different cell-based search spaces. Unfortunately, there exists no similar large-scale benchmark for chain-like search spaces at the moment.

However, to also shed some light on these types of search spaces, we added an experiment to the revised paper where we leverage a reduced version of the NASBench-101 search space to create a chain-like search space. We re-ran our experiments on this space and present the results in Appendix A of the revised paper. Our findings also hold in this case.

\mypara{Q2.} \textit{In Section 4, are the three random initialization using the same three seeds as the three seeds of the three runs in the original NASBench-101?}

\mypara{Reply:} We ensure that the architectures are initialized identically to the original runs in NASBench-101. Note that, as the original NASBench-101 uses a Tensorflow implementation  and we conducted our experiments in PyTorch, small differences in layer implementations render simply using the same random seeds not sufficient to ensure that all parameters are initialized identically. We thus used Tensorflow to initialize the parameters and copied the resulting parameters into our PyTorch implementation. We added a note in Section 4 to make this clear.

\mypara{Q3.} \textit{How do you compute the correlation between S-KdT and final performance/super-net accuracy in Fig.6 and Table 3? S-kdT is a scalar given two ranked lists, while final performance/super-net accuracy is a vector (i.e., a list of scalar numbers). How do you calculate the correlation between a scalar and a vector? Please explain this to me, or point out that I misunderstand it. BTW, it would be better to clarify this in the paper. }

\mypara{Reply:} There seems to be a misunderstanding related to the definition of super-net accuracy and final performance. Section 3.2.1, second paragraph, defines super-net accuracy: `... super-net accuracy, we report the \underline{average accuracy} of 200 architectures on the validation set ...'. As such this is one scalar per independent run. In the same section, third paragraph, we define final performance as `... the stand-alone accuracy of \underline{the model that was found by the complete WS-NAS algorithm} ...'. This a single final architecture with one scalar performance value. As such, for each independent super-net training run, \skdt, final performance, and super-net accuracy are all scalars. Multiple independent runs thus create the same number of metrics for each of these three quantities, and we can directly correlate them. We revised the captions to clarify this.


\mypara{Q4.} \textit{In page 9, Section 4.4, the 3rd paragraph, ".Table 4 shows 
that this decreases the sparse Kendall-Tau from 0.7 to 0.5. 
". However, in Table 4, the ''Init Channel" block does not decrease S-KdT from 0.7 to 0.5, actually from 0.74 to 0.69. Moreover, "but one 
can reduce the batch size by a factor > 0.5 and use only one 
repeated cell." However, in Table 4, the "Repeated Cells" block suggests that reducing repeated cells decreases the S-KdT from 0.75 to 0.50. I am confused by the context here and the results in Table 4. Are they misplaced? 
}
\mypara{Reply:} The original text swapped the `Init channel' and `Repeated cells', and we revised the text to correct this. 

\mypara{Q5.} \textit{It really confuses me when I try to understand Table 5. More direct explanations of the "Baseline, Baseline-v2, Ours" should be given to ease the reading.}

\mypara{Reply:} Baseline-v2 disables the dynamic channels during the test phase only, in contrast to the Baseline where dynamic channels are enabled during both the training and test phase. We revised the text and moved these results to a new table named ablation study.


==> tex/R2.tex <==
\section{Reviewer 2}

\mypara{Q1.} \textit{This submission lacks the ImageNet results for the comparison w.r.t. other NAS approaches. }

\mypara{Reply:} Conducting our analysis on ImageNet is unfortunately not possible due to the heavy computation requirement and the lack of tabular benchmark spaces for ImageNet. \ky{For example, to construct the DARTS-NDS space on ImageNet, we need to train 5000 architectures on ImageNet, which roughly takes 20,000 GPU days.}

\mypara{Q2.} \textit{The authors studied 14 heuristics, while in Sec.5, only 5 are useful. That makes others look useless. }

\mypara{Reply:} We believe that this is a core contribution of our analysis. We reveal that, contrary to popular belief, many commonly used techniques actually negatively impact search performance. As a consequence, NAS practitioners can focus on the useful heuristics in the future. 

\mypara{Q3.} \textit{In many existing works, they have claimed the same statement. From this point, the contribution of this manuscript lies in a deep analysis of existing training strategies. At the current stage of NAS, it might not be enough for a TPAMI submission. }

\mypara{Reply:} We for the first time comprehensively compare different factors that influence NAS performance under a common and fair experimental protocol. Previous works did not report or provide detailed analyses of these factors as they understandably focus on their own proposed NAS search algorithms. The fact that only a few of the tested factors actually prove useful is a testament for the need for such an analysis.

\mypara{Q4.} \textit{If I remember correctly, the limitation of page numbers for the first submission is 12? If so, this submission needs to be trimmed a little bit. }

\mypara{Reply:} The TPAMI author guidelines\footnote{\url{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8000767}} state a page limit of 18 pages for regular papers.




==> tex/R3.tex <==
\section{Reviewer 3}

\mypara{Q1.} \textit{First issue is Fig1,2 contains too much concepts. Perhaps we should emphasis more on the difference so that the main information could be clearly delivered. }

\mypara{Reply:} Thank you for this suggestion. We have simplified the figures and updated the captions to make the differences between the concepts more clear.

\mypara{Q2.} \textit{Another issue resides in Fig4 where the author says: 'Fig. 4: Ranking disorder examples. We randomly select 12 runs from our experiments. For each sub-plot, 0 indicates the architecture ground-truth rank, and 1 indicates the ranking according to their super-net accuracy. We can clearly see that the ranking disorder happens uniformly across the search space and does not follow a particular pattern'. However, I think this claim could not be fully supported by the evidence. }

\mypara{Reply:} We agree that this statement as such was not sufficiently supported by evidence. We toned down this claim by deleting `the disorder happens uniformly'.

\mypara{Q3.} \textit{Finally in Table 10, it could be seen that, for different hyper parameter setting and benchmark, the final performance is deviating from the correlation metric. It would be very interesting if the result is repeatable. I would suggest looking into the correlation of different ranking group eg.(rank 1-10 rank 11-20 rank 21-30 might have different correlation behaviour). This is very important because of the nature of searching algorithm would probably let high-ranking(better) affect the final performance more. }

\mypara{Reply:} 
% We are not entirely sure to understand the reviewer's question. 
Our sparse Kendall Tau metric already considers groups of architectures. For example, if the rank 1-10 architectures only differ by 0.01\% top-1 accuracy, and the ranking of these architectures is randomly permuted, our sparse Kendall Tau will yield a correlation of 1, which indicates a perfect ranking.  
Note that, to train the super-net, we chose the widely-used single-path one-shot algorithm, which uniformly randomly samples one architecture during the entire super-net training phase. The search is then conducted on a trained super-net and hence does not update the super-net weights. As such, it cannot further affect the behavior of the high-ranking architectures.
%It's unlikely the search algorithms push higher ranking group to behaive better. 
This is also indicated by Figure 4, which shows no obvious pattern related to architecture groups, revealing that the search algorithms do not positively affect high-ranking architectures. 

% \mypara{Q4.} \textit{Across all the paper, experiments is conducted 3 times. There is a chance that this is not sufficient. Inspire of that, I am convinced by the experiments in the paper, which reveals the noisy nature of training and evaluation of DNNs. }

% \mypara{Reply:} Due to the computation budget, repeating 3 times is the maximum budget that we can afford, which led to a total cost of 600 GPU days of computation. Nonetheless, repeating each experiments for three times is a thumb of rule in current research communities. We nonetheless thank the trust of the reviewer.



==> tex/exp-extra.tex <==

\section{Results for other factors}
\label{apdx:additional-result}
Here, we discuss the results of the remaining factors. 

\subsection{Weight-sharing Protocol $P_{ws}$ -- Other Factors}
\label{apdx:wsp}

% We report results of additional factors such as the number of training epochs, weight decay \ky{and path sampling} here. In summary, our experiments show that more training epochs 
% positively influence super-net quality. 
% The behavior of weight decay varies across datasets, and one cannot simply disable it as suggested by~\cite{nayman2019xnas}.
% 
% 
% \input{figure/lr-other-spaces.tex}


% Traditionally, accuracy across epochs is represented as a line plot, where the data points on the same line are obtained in a sequential order and with to the same training procedure
% . However, because the cosine learning rate scheduler decays the learning rate to 0, the loss decay is also quite smooth. \MS{I don't get this.}
% In our scenario, each data point on the line represents the individual training at a target epoch over 3 different runs. 


% \subsection{Weight-sharing Protocol $P_{ws}$ -- Path Sampling}

% We further validate the different implementations of the core layers in the mapping function $f_{ws}$. We analyze the dynamic channeling in detail and evaluate other mapping factors in Appendix~\ref{apdx:fws-other}. 


% Furthermore, as evidenced by \Figref{fig:disable-channel-result}, where we plot the \skdt{} across the epochs,
%for both the baselines and the new dynamic channeling \MS{new or disabled?}, 
% \ms{disabling dynamic channelling} greatly improves training stability.




\subsection{Mapping \fws{} -- Other Factors}
\label{apdx:fws-other}


==> tex/revision.tex <==
We would like to thank the associate editor and the reviewers for their effort on improving the quality of this submission. We have revised and improved the work based on all the comments and the suggestions.
We first provide a ``Revision summary" in Section~\ref{sec:summary} to list the key differences between the previous submission and the revision. We then provide detailed responses to each reviewer in the following sections. 

\section{Revision summary}
\label{sec:summary}

\begin{enumerate}
    \item We provide additional experiments for a chain-like search space. To this end, because there exist no benchmark linear search space, we leverage the NASBench-101 search space to construct a chain-like linear space and repeat our analysis in Appendix A.
    \item We revised our paper according to the reviewers suggestions. A version of our manuscript with highlighted changes is attached as supplementary material. Additions are highlighted in \changed{blue}, whereas deletions are highlighted as \removed{red strike-through text}.
\end{enumerate}



